Computing Generalized Convolutions Faster Than Brute Force

In this paper, we consider a general notion of convolution. Let $D$ be a finite domain and let $D^n$ be the set of $n$-length vectors (tuples) of $D$. Let $f : D \times D \to D$ be a function and let $\oplus_f$ be a coordinate-wise application of $f$. The $f$-Convolution of two functions $g,h : D^n \to \{-M,\ldots,M\}$ is $$(g \otimes_f h)(\textbf{v}) := \sum_{\substack{\textbf{v}_g,\textbf{v}_h \in D^n\\ \text{s.t. } \textbf{v}_g \oplus_f \textbf{v}_h}} g(\textbf{v}_g) \cdot h(\textbf{v}_h)$$ for every $\textbf{v} \in D^n$. This problem generalizes many fundamental convolutions such as Subset Convolution, XOR Product, Covering Product or Packing Product, etc. For arbitrary function $f$ and domain $D$ we can compute $f$-Convolution via brute-force enumeration in $\widetilde{O}(|D|^{2n}\mathrm{polylog}(M))$ time. Our main result is an improvement over this naive algorithm. We show that $f$-Convolution can be computed exactly in $\widetilde{O}((c \cdot |D|^2)^{n}\mathrm{polylog}(M))$ for constant $c := 3/4$ when $D$ has even cardinality. Our main observation is that a \emph{cyclic partition} of a function $f : D \times D \to D$ can be used to speed up the computation of $f$-Convolution, and we show that an appropriate cyclic partition exists for every $f$. Furthermore, we demonstrate that a single entry of the $f$-Convolution can be computed more efficiently. In this variant, we are given two functions $g,h : D^n \to \{-M,\ldots,M\}$ alongside with a vector $\textbf{v} \in D^n$ and the task of the $f$-Query problem is to compute integer $(g \otimes_f h)(\textbf{v})$. This is a generalization of the well-known Orthogonal Vectors problem. We show that $f$-Query can be computed in $\widetilde{O}(|D|^{\frac{\omega}{2} n}\mathrm{polylog}(M))$ time, where $\omega \in [2,2.372)$ is the exponent of currently fastest matrix multiplication algorithm.

==> Makefile <==
SOURCES := $(shell find $(SOURCEDIR) -name '*.tex')

all: main.pdf

main.pdf: $(SOURCES) main.bbl 
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: bib.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/cut-and-count-diff/
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d2.tex
	git checkout $(branch-id)
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d1.tex
	latexdiff /tmp/cut-and-count-diff/d1.tex /tmp/cut-and-count-diff/d2.tex > /tmp/cut-and-count-diff/diff.tex
	pdflatex /tmp/cut-and-count-diff/diff.tex
	git checkout master


==> genconv.tex <==
\section{Generalized Convolution}
\label{sec:gen-convolution}


\karol{We need to discuss where this goes}
\ariel{there is a text duplication here we need to resolve.}

For any $k\in \Nat$, let $\Int_k=\{0,1,\ldots, k-1\}$.
We say a function $f: A\times B\to C$ is {\em $k$-cyclic}
if, up to a relabeling of the sets $A$, $B$ and $C$,
it is an addition modulo $k$.
Formally, $f: A\times B\to C$ is {\em $k$-cyclic}
if there are $\sigma_A:A\to\Int_k$,
$\sigma_B:B\to\Int_k$,
and $\sigma_C: \Int_k \to C$ such that
\[
  \forall a\in A, ~b\in B:~~~f(a,b) = \sigma_C\left( \sigma_A(a)+ \sigma_B(b)\mod k\right)
  .
\]
We refer to the functions $\sigma_A$, $\sigma_B$ and $\sigma_C$ as the {\em relabeling} functions of $f$. 

The {\em restriction} of $f: L\times R \to T$ to $A\subseteq L$ and $B\subseteq
R$ is the function $\tilde{f}:A\times B\to T$ defined by $\tilde{f}(a,b) =
f(a,b)$ for all $a\in A$ and $b\in B$.  We say $(A,B,k)$ is a {\em cyclic minor}
of $f: L\times R \to T$ if the restriction of $f$ to $A$ and $B$ is a $k$-cyclic
function.

A {\em cyclic partition} of $f: L\times R \to T$
is a set of minors $\cM=\{(A_1,B_1,k_1),\ldots, (A_m,B_m,k_m)\}$
such that $(A_i,B_i,k_i)$ is a cyclic minor of $f$
and for every $(x,y)\in L\times R$ there is a unique  $1\leq i\leq m$
such that $(x,y)\in A_i\times B_i$.
The cost of the cyclic partition is $\cost(\cM)=\sum_{i=1}^m k_i$.

Observe that a minor $(A_i,B_i,k_i)$ explicitly determines set $C_i$ of the
domain, i.e., $f(A_i,B_i) = C_i$. \ariel{Do we really need the set $C_i$? I think we can avoid it}


\begin{lemma}
	\label{lem:fastConvolutionUsingMinor}
  Let $L$, $R$ and $T$ be finite sets.
  Also, let $f:L\times R\to T$ be a function
  and let $\cM$ be a cyclic partition of $f$.
  Then there is an $\Os(\cost(\cM)^n)$ algorithm for \fConv.
\end{lemma}

\begin{lemma}
	\label{lem:existenceOfMinor}
	Let $f:L\times R\to T$ where $L$, $R$ and $T$ be finite sets.
  Then there is a cyclic partition $\cM$ of $f$ such that
  \[
    \cost(\cM)\leq
      \begin{cases}
        \frac{\abs{L}}{2} \cdot \frac{4\cdot \abs{R} + \abs{T}}{3} &
          \abs{L} \text{ is even} \\
        \abs{R} + \frac{\abs{L}-1}{2} \cdot \frac{4\cdot \abs{R} + \abs{T}}{3} &
          \abs{L} \text{ is odd}
      \end{cases}
    .
  \]
\end{lemma}

